Local clustering of relic neutrinos: Comparison of kinetic field theory and the Vlasov equation

Gravitational clustering in our cosmic vicinity is expected to lead to an enhancement of the local density of relic neutrinos. We derive expressions for the neutrino density, using a perturbative approach to kinetic field theory and perturbative solutions of the Vlasov equation up to second order. Our work reveals that both formalisms give exactly the same results and can thus be considered equivalent. Numerical evaluation of the local relic neutrino density at first and second order provides some fundamental insights into the frequently applied approach of linear response to neutrino clustering (also known as the Gilbert equation). Against the naive expectation, including the second-order contribution does not lead to an improvement of the prediction for the local relic neutrino density but to a dramatic overestimation. This is because perturbation theory breaks down in a momentum-dependent fashion and in particular for densities well below unity.

==> Born-approximation.tex <==
% !TEX root = main.tex

\section{Kinetic field theory: Born approximation}

The formal solution of the equations of motion in eq.~\eqref{eq:formal_solution} is of little direct use, as it requires the integration over the derivative of the gravitational potential \textit{along the trajectory}. Remedy can be provided by the \textit{Born approximation}, where the integration is instead performed along the \textit{free trajectory}, i.e.
\begin{align}
    \vec{x}^{\,s}(z) \approx & \restr{\vec{x}^{(i)} + g(z,z_i) \vec{p}^{(i)} + m_{\nu} \int_{z_i}^z \mathrm{d}z' \, \frac{g(z,z')}{(1+z') H(z')} \frac{\partial \varphi(\vec{x}(z'))}{\partial \vec{x}} }{\Vec{x}(z')=\vec{x}^{(i)}+g(z',z_i)\vec{p}^{(i)}} \\
    =& \restr{\vec{x}^{(i)} + g(z,z_i) \vec{p}^{(i)} + m_{\nu} \int_{z_i}^z \mathrm{d}z' \, \frac{g(z,z')}{(1+z') H(z')}   \vec{x}(z') R_1(r(z'))}{\Vec{x}(z')=\vec{x}^{(i)}+g(z',z_i)\vec{p}^{(i)}} \, ,
    \label{eq:trajectory_Born}
\end{align}
where $r(z')=|\vec{x}(z')|$. \IO{Need to shift the definition of the $R_1$, $R_2$ and $R_3$ functions from sec. \ref{sec:Kinetic field theory: Perturbative approach} to here...}
In the context of structure formation it has been shown that this approximation performs best for trajectories that deviate slightly from free trajectories [CITE?]. We therefore expect it to be reasonably well for high momenta and low neutrino masses $m_{\nu}$. 

For a spherically symmetric gravitational potential the derivative with respect to the initial positions $x^{(i)}_j$ can then be written as

\begin{align}
    \frac{\partial x_i(z)}{\partial x^{(i)}_j}  =& \delta_{ij} +    m_{\nu}\int_{z_i}^z \mathrm{d}z' \, \frac{g(z,z')}{(1+z')H(z')} \left( \delta_{ij} R_1(r(z')) + x_i(z') x_j(z') \, R_2(r(z')) \right)    \Bigg|_{\vec{x}(z')=\vec{x}^{(i)}+g_(z',z_i)\vec{p}^{(i)}} 
\label{eq:derivatives1}
\end{align} 
which we can write as
\begin{align}
    \frac{\partial x_i(z)}{\partial x^{(i)}_j}  \ec & \delta_{ij}  + \delta_{ij}I_1  + x_i^{(i)} x_j^{(i)} I_{xx} + \left( p_i^{(i)} x_j^{(i)} + x_i^{(i)} p_j^{(i)} \right) I_{xp} + p_i^{(i)} p_j^{(i)} I_{pp} \, .  
    \label{eq:derivative_Born}
\end{align} 
%
The integrands in the above equation are defined as 
\begin{align}
    I_1 &= \restr{m_{\nu} \int_{z_i}^z \diff z' \frac{g(z,z')}{(1+z')H(z')} R_1(r(z'))}{\Vec{x}(z')=\vec{x}^{(i)}+g(z',z_i)\vec{p}^{(i)}}\\
    I_{xx}  &= \restr{m_{\nu} \int_{z_i}^z \diff z' \frac{g(z,z')}{(1+z')H(z')} R_2(r(z'))}{\Vec{x}(z')=\vec{x}^{(i)}+g(z',z_i)\vec{p}^{(i)}}\\
    I_{xp} &= \restr{ m_{\nu} \int_{z_i}^z \diff z' \frac{g(z,z') \, g(z',z_i)}{(1+z')H(z')} R_2(r(z'))}{\Vec{x}(z')=\vec{x}^{(i)}+g(z',z_i)\vec{p}^{(i)}} \\
    I_{pp} &= \restr{m_{\nu} \int_{z_i}^z \diff z' \frac{g(z,z') \, g(z',z_i)^2}{(1+z')H(z')} R_2(r(z'))}{\Vec{x}(z')=\vec{x}^{(i)}+g(z',z_i)\vec{p}^{(i)}} \, .
\end{align}
Eq. \eqref{eq:derivatives1} can now be used in order to find an expression for the determinant appearing in the local relic density \eqref{eq:number_density_exact}  \IO{Changed the notation here, I think there will be a few extra terms in the following. However, I guess there is not even any need to write the determinant out explicitly... Probably eq. \eqref{eq:derivative_Born} is sufficient...} ,
\begin{align}
&\mathrm{det} \left( \frac{\partial{\vec{x}(z_0})}{\partial{\vec{x}^{(i)}}} \right)_{\vec{x}(z_0)=\vec{x}_0,\vec{y}^{(i)}}= I_1^3+I_1^2 \left(I_{pp} \,\norm{\vec{p}^{(i)}}^2 + 2 I_{xp} (p_1^{(i)} x_1^{(i)}+p_2^{(i)} x_2^{(i)}+p_3^{(i)} x_3^{(i)}) +  I_{xx} \,\norm{\vec{x}^{(i)}}^2 \right)  \\
&- I_1 \left(I_{xp}^2-I_{pp} I_{xx}\right) \left({p_1^{(i)}}^2 \left({x_2^{(i)}}^2+{x_3^{(i)}}^2\right)+{p_2^{(i)}}^2 \left({x_1^{(i)}}^2+{x_3^{(i)}}^2\right)+{p_3^{(i)}}^2 \left({x_1^{(i)}}^2+{x_2^{(i)}}^2\right) \right. \\
&\left. -2 p_2^{(i)} x_2^{(i)} p_3^{(i)} x_3^{(i)} - 2 p_2^{(i)} x_2^{(i)} p_1^{(i)} x_1^{(i)} - 2 p_1^{(i)} x_1^{(i)} p_3^{(i)} x_3^{(i)}\right) \, .
\end{align}

\IO{In order to evaluate the determinant in eq. \eqref{eq:number_density_exact} we need to numerically find the initial positions $x^{(i)}_i$ which fulfill $\vec{x}^{\,s}(z)=\Vec{x}$ applying \eqref{eq:trajectory_Born} for given $\Vec{p}^{(i)}$. }

\subsection{Method}
